Memory-efficient Sketch Acceleration for Handling Large Network Flows on FPGAs

Sketch-based algorithms for network traffic monitoring have drawn increasing interest in recent years due to their sub-linear memory efficiency and high accuracy. As the volume of network traffic grows, software-based sketch implementations cannot match the throughput of the incoming network flows. FPGA-based hardware sketch has shown better performance compared to software running on a CPU when handling these packets. Among the various sketch algorithms, Count-min sketch is one of the most popular and efficient. However, due to the limited amount of on-chip memory, the FPGA-based count-Min sketch accelerator suffers from performance drops as network traffic grows. In this work, we propose a hardware-friendly architecture with a variable width memory counter for count-min sketch. Our architecture provides a more compact design to store the sketch data structure effectively, allowing us to support larger hash tables and reduce overestimation errors. The design makes use of a P4-based programmable data plane and the AMD OpenNIC shell. The design is implemented and verified on the Open Cloud Testbed running on AMD Alveo U280s and can keep up with the 100 Gbit link speed.

==> analysis.tex <==
To achieve high throughput, the hardware designs of count-min sketch (with or without conservative updates) are built with pipeline architectures. However, pipeline architectures often encounter data hazards, which can lead to a decrease in performance and may even impact the correctness of the design. 
%
In this section, we analyze the potential data hazards of the hardware architecture of different Count-Min sketch algorithms.
We discuss the undesirable effects caused by these hazards and then provide an alternative solution. 


\begin{figure}[ht]
    \center
    \includegraphics[scale=1,width=\linewidth]{figures/normal_ppl.pdf}
    \caption{\label{fig:normal_ppl}Single Data in the Pipeline}
  \end{figure}
  
\paragraph{Data Hazard and Effects} Fig.~\ref{fig:normal_ppl} illustrates the status of a single element inside a general count-min pipeline architecture as a function of time. For a single data item, its corresponding counter value is successfully committed to memory and ready to be read again after $(R+C+W)$ cycles, where $R$ and $W$ stand for the memory read and write latency in cycles, and the $C$ is the latency for calculating the updated value. During
these cycles, the pipeline continues to issue reads for successive data items.

A data hazard occurs if any of the successive data items issues a memory read to the same counter location as the current item during the next $(R+C+W)$ cycles.

\begin{figure}[ht]
    \center
    \includegraphics[scale=1,width=\linewidth]{figures/ppl.pdf}
    \caption{\label{fig:ppl}Pipeline Illustration of Count-Min Sketch. Data synchronizations are allowed at DFU but not at update value stage.}
  \end{figure}

Most existing designs use a Data Forwarding Unit (DFU), constructed with shift registers to resolve the data hazards. This pipeline is shown in Fig.~\ref{fig:ppl}.  This architecture keeps track of the counter values of the current packet's successors. These values will be directly synchronized with the latest committed counter values if they share the same key. Thus, the DFU 
 will resolve any data hazards. 

However, the data hazard scenario becomes more complicated when the conservative update algorithm is used. 
The update block will find the minimum values of all counter values from the previous memory read blocks. Finding the minimum values from multiple candidates requires multiple stages with data dependence in between.  
The minimum value must be recalculated when any counter values are updated. 
The update block will no longer produce the minimum value in constant $C$ cycles.
Therefore, it is infeasible to implement a DFU for the data hazards that arise due to conservative updates as in Fig.~\ref{fig:ppl}.

In the existing work on CM-CU hardware design~\cite{soto2021high}, the data hazards of the update block are ignored.
The authors claim that since the update block has a small number of stages, ignoring the data hazards will not primarily affect the algorithm's accuracy.
However, an essential property of the count-min sketch is its one-sided error. 
As the counter values always increase for every data item, 
the sketch algorithm only overestimates the 
size of the data elements but not underestimate any item.
It guarantees the results of the algorithm are no smaller than their true values.
Yet, failing to maintain the data consistency between the pipeline stages and memory will cause a decrease in counters eventually.
Therefore, the count-min sketch with conservative update can no longer guarantee the one-sided error. We use real world network traces to evaluate the design ignoring data hazards. The design returns a 5\% false negative rate (which is an underestimation), rather than
0. Detailed results are shown in Section~\ref{subsec:experiment}.

To mitigate the impact of data hazards, we categorize the conflicts into two kinds: false conflicts and true conflicts.
A false conflict is where the conflicting items are in fact identical.
Packets that arrive in a consecutive order during a short period likely belong to the same flow, which results in false conflicts.
In the case of a true conflict, the data elements are not the same but generate the same hash value in at least one hash table. The limited size of the counter tables causes true conflicts. Targeting these two types of conflicts, we propose two methods to eliminate or prevent data hazards, as described in the following sections. 

\paragraph{Merging}

False conflict should not result in a collision pair. 
As the order of the stream sequence will not affect the overall estimation, the sketch data is mergeable~\cite{agarwal2013mergeable}.
We can merge the same items into a single entity.
Input items are buffered before entering count-min sketch. 
The latest item will compare its key with all buffered items, and 
merge with elements with the same key.  
If we define the buffer depth as $L$, the merging guarantees no false conflicts exist for any consecutive $L$ elements. 

\paragraph{Hybrid Update for Hardware Architecture}

We propose
a heuristic-based hybrid update strategy combining conservative and original updates to handle the true conflicts. 
For each data item entering the update block, we use a hazard detection unit to look through all the elements in the update block and identify any conflicts with the current item. If a conflict is detected, instead of using
a conservative update, we applied the original update as described in Algorithm~\ref{alg:cm} for this item. 
Although the traditional update increases the rate of over-estimation compared to the conservative update, it can achieve similar performance to conservative update methods.   
This strategy mostly benefits from the conservative update and also avoids the pipeline hazard issue it introduces. 
Throughout this paper, we refer to our update strategy as the \emph{hybrid} strategy.
